Ultra-high Resolution Image Segmentation via Locality-aware Context Fusion and Alternating Local Enhancement

Ultra-high resolution image segmentation has raised increasing interests in recent years due to its realistic applications. In this paper, we innovate the widely used high-resolution image segmentation pipeline, in which an ultra-high resolution image is partitioned into regular patches for local segmentation and then the local results are merged into a high-resolution semantic mask. In particular, we introduce a novel locality-aware context fusion based segmentation model to process local patches, where the relevance between local patch and its various contexts are jointly and complementarily utilized to handle the semantic regions with large variations. Additionally, we present the alternating local enhancement module that restricts the negative impact of redundant information introduced from the contexts, and thus is endowed with the ability of fixing the locality-aware features to produce refined results. Furthermore, in comprehensive experiments, we demonstrate that our model outperforms other state-of-the-art methods in public benchmarks. Our released codes are available at: https://github.com/liqiokkk/FCtL.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> imgs/methods/method_421.tex <==
\section{Our Proposed Methodology}
\label{sec:method}
\subsection{Overview}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{imgs/steps.png}
    \caption{Main procedure of high-resolution image segmentation, consisting of (i) cropping local patches from the ultra-high resolution image; (ii) local patch segmentation; (iii) merging local masks into a high-resolution mask.}
    \label{fig:steps}
\end{figure}

Our proposed ultra-high resolution image segmentation framework follows the three-step procedure as shown in Fig. \ref{fig:steps}, which is consistent with the common practice applied in prior works (e.g., \cite{ronneberger2015u,chen2019collaborative}). 
% We first sample or crop several local patches from the input image, then compute the segmentation result for each patch, and combine the local segmentation into one piece as the final result. 
First, given an ultra-high resolution image $\dot{I}$ with width $W$ and height $H$, we evenly partition it into $N$ local patches $\{I_{k}\}$ ($k=[1,\cdots,N]$, $I_{k} \subset \dot{I}$) with width $w$ and height $h$ ($w<W$ and $h<H$). 
% In practice, the adjacent patches are partially overlapped. 
Next, a local semantic segmentation model computes the local result for each patch. Last, we merge the local results into one piece as the final high-resolution segmentation mask. 
% In this step, we replace the trivial merging approach with a semantics refinement network to refine the local masks.
% i.e., $\dot{M} = \mathcal{F}_{merge}(M_1,\cdots,M_N)$. 
Our main contributions rest in how to generate fine local segmentation. As follows, we will elaborate the technical details. 





% $\{\{I_{ij}\}_{j=1}^{n}\}_{i=1}^{N}$ with N scales and the different scales of each patch have the same center point. The segmentation branch receives $I_{1j}$ and the contextual branch receives $I_{ij},i \in [1,...,N]$ for patch $j$(see example). Note that $I$ is fully cropped into patches(instead of random cropping)to facilitate both training and inference. $I_{ij} \in \mathbb{R}^{h \times w}$, where $h \ll H$, and $w \ll W$. We adopt the same backbone for two branches and xxx Module acts on deep feature.


% \subsection{Our Proposed Local Segmentation Model}

\begin{figure*}
    \centering
    % \includegraphics[width=0.95\textwidth]{imgs/framework4.png}
    \includegraphics[width=0.95\textwidth]{imgs/framework.png}
    \caption{Illustration of our local segmentation model. In specific, a certain local patch cropped from the high-resolution image and its contexts are passed into the network branches separately to extract features and then measure their relevances against local patch to obtain the locality-aware features and adaptively fused via the Locality-aware Context Fusion Module (LCFM). On the other hand, the local regions of  contextual features are upsampled and mutually optimized to yield robust local representation via the Collaborative Local Representative Optimization Module (CLROM) for producing high-quality local segmentation results.}
    \label{fig:framework}
\end{figure*}

As the core of our ultra-high resolution segmentation framework, we propose a novel local segmentation model to process each cropped patch (Fig.~\ref{fig:framework}).
% It is obvious that the quality of local patch segmentation affects the final segmentation result of the ultra-high resolution image. 
Yet, each local patch only covers a confined field of the ultra-high resolution image, which often contains regions of varied scales or truncated objects, and thus it tends to deliver incomplete information and may easily cause erroneous semantic segmentation. 
% it is difficult to infer the contextual and holistic information on image content. 
% Specifically, the object of interest (e.g. building) may be truncated, and thus confuse the local segmentation model for inferring its semantic meaning. 
% Inspired by prior practices \cite{chen2019collaborative}, involving contextual information relevant to the local patch during inference can be effective to mitigate the problems. 
To address this concern, we propose a locality-aware contextual correlation based segmentation model for processing each local patch.
% Hence, we propose a context-aware local segmentation model that can well exploit the image context without increasing too much computation burden. 
% to introduce the contextual information of a local patch to enhance the local segmentation. 

As illustrated in Fig. \ref{fig:framework}, our local segmentation model is based on a multi-stream encoder-decoder architecture, consisting of the feature extraction modules (i.e., encoder), locality-aware context fusion module (LCF), alternating local enhancement module (ALE), and decoder. In specific, an image patch and its context regions of different scales, which are rescaled into the same size for reducing computation overhead, are fed into the network for feature extraction. Then, the features of contexts are separately associated with the features of local patch via two proposed modules, LCF and ALE, to strengthen the local features. In final, the enhanced local features will be upsampled and decoded to obtain the local segmentation mask. 
As follows, we will first introduce how to choose the context of local patch, and then describe the proposed modules, respectively. 

% Hence, our local segmentation model mainly consists of two components: local-context relevance module and multi-scale context fusion scheme.
% As follows, we will first define the context of the local patch and then introduce our proposed local-context relevance module to attentively strengthen the visual features of local patches. Last, we present how to adaptively fuse multi-scale context to improve the local segmentation.



\subsection{Context of Local Patch} 
\label{sec:choose_context}

% Assume that the entire ultra-high resolution image $\dot{I}$ is equally divided into $K$ patches. 
Amongst all $N$ patches, regarding of the $k$-th patch $I_k$, $U_k$ is denoted as another image region within $\dot{I}$, which is not smaller than and covers $I_k$. $U_k$ has the width $w_u$ and height $h_u$, s.t. $w \leq w_u \leq W \text{ and } h \leq h_u \leq H$. 

Given a local patch, there are many candidate context regions. In practice, we design the following three types of context regions. (1) We set the size of the candidate context subject to $w_u = \lambda w \text{ and } h_u = \lambda h, (\lambda \geq 1, w_u \leq W, h_u \leq H)$, and its center aligned with the center of the local patch (see the examples in Figs.~\ref{fig:teaser} and ~\ref{fig:framework}). (2) The largest context we can utilize is exactly the whole image, i.e., $U_k \equiv \dot{I}$, dubbed \textit{global context}. (3) The smallest context is the patch itself, dubbed \textit{local context}, i.e., $w_u \equiv w \text{ and } h_u \equiv h$. 
Generally, the larger contexts offer more contextual cues that may be responsible for large regions or objects, while the smaller ones provide more details that may be attributed to small regions or objects. Before feeding the contexts along with local patch into network, they will be rescaled as the same dimension as the local patch in order to reduce the computation overhead.

% For the scale of the context region, there are several cases to consider: (1) $w_u \equiv w, h_u \equiv h$: The smallest context region is the local patch itself. In this case, measuring local-context relevance is essentially the evaluation of self-correlation, which is effective since certain regions within the patch may help identify other regions. (2) The context region matches the entire image, i.e., $U_k \equiv \dot{I}$: In this case, the entire image can provide the holistic information. (3) $w < w_u < W, h < h_u < H$: 
% Most selected context regions are larger than the local patch while smaller than the entire image. 
% Generally, the larger contexts offer more global cues, while smaller ones provide more details. 
% In practice, we let the center of the selected context regions to be aligned with the center of the local patch.
% Additionally, we choose the contexts with the identical aspect ratio with the local patch and normalize them into the same dimension as the local patch before feeding them into the network. 

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.9\textwidth]{imgs/local.png}
    \caption{...}
    \label{fig:local_framework}
\end{figure*}

\input{lcf}

\subsection{Locality-aware Context Fusion}

% Formally, we define a context region of the $k$-th local patch $I_k$ as $U_k$. 
To strengthen the segmentation of a local patch, we would like to associate the contextual information with the local information. Thus, as illustrated in Fig.~\ref{fig:framework}, we propose the LCF module $\mathcal{F}_{LCF}$ to evaluate the relevance between the features of $I_k$ and $U_k$, and then utilize it to obtain its locality-aware features. 
The structure of our produced module is specified in the left figure of Fig.~\ref{fig:local_framework}. It mainly consists of two steps: locality-aware contextual correlation (LCC) and multi-context fusion (MCF). Specifically, LCC discovers the relevance of local patch and contexts to enhance local features, and MCF then adaptively merges them so the contexts can well complement the local features. 



\subsubsection{Locality-aware Contextual Correlation}
% \textcolor{red}{[Motivation and aim of LCC block]}
% In LCC block, we aim to correlate the contexts and local patches. 
\wx{Inspired by the recent development in vision transformers~\cite{dosovitskiy2021an}, we want to capture the positional relevance of local patch and contexts to enhance local patch. To accomplish this purpose, we propose the following procedure.}
First, the features of $I_k$ and $U_k$ are separately extracted through the identical yet independent backbone network structures (e.g., Conv1 to Conv3 of the pretrained VGG16~\cite{Simonyan15} \wx{or pretrained Segformer~\cite{xie2021segformer}).}
For the sake of simplicity in description, we omit the subscript $k$ below. Hence, the extracted features can be denoted as $\textbf{X}^I$ and $\textbf{X}^U$ ($\textbf{X}^I,\textbf{X}^U \in \mathbb{R}^{c \times h_x \times w_x}$). 

Next, the relevance of $I$ and $U$ is calculated via the inner product of local features $\textbf{X}^I$ and contextual features $\textbf{X}^U$, i.e., $\textbf{R} = \langle\textbf{X}^I,\textbf{X}^U \rangle$, which measures the non-local correlation by establishing the pairwise pixel-level relation for $\textbf{X}^I$ and $\textbf{X}^U$, as illustrated in the left figure of Fig.~\ref{fig:local_framework}.
Hence, the relevance can be further applied as an attention map to enhance the local features, $\textbf{X}^I$, which attends to the semantic regions more relevant with the locality. 
% Specifically, $\textbf{R}_k$ is passed through a softmax layer to obtain the attention map and then perform element-wise multiplication with $\textbf{X}_k^i$, i.e., $\overline{\textbf{X}_k} = \text{Softmax}(\textbf{R})_k \odot \textbf{X}_k^i$.
\textcolor{blue}{Specifically, $\textbf{R}$ is passed through a softmax layer to obtain its corresponding attention map as below: 
\begin{align}
    M=\text{Softmax}(\textbf{R}) = \text{Softmax}(\langle\textbf{X}^I,\textbf{X}^U \rangle).
    \label{eq:m_k1}
\end{align}}
% Then, we perform inner product with $\textbf{X}_k^U$, i.e., $\overline{\textbf{X}}_k = \langle M_k , \textbf{X}_k^U\rangle$.
% Last, $\overline{\textbf{X}}_k^i$ will be utilized to achieve the segmentation result $M_k$. 
% For the sake of clarity, we denote the entire procedure as $\overline{\textbf{X}}_k = \mathcal{F}_{lcc}(I_k, U_k)$.


% Overall, the inference process of the $k$-th local patch segmentation with regards to its certain context region can be expressed as below:
% \begin{align}
%     M_k &= \mathcal{F}_{seg}(I_k,U_k),\nonumber\\
%     &= F_{up}(F_{lcr}(F_{fe}(I_k), F_{fe}(U_k))).
% \end{align}

% To  enhance local branch deep feature, we introduce a xxx module. The xxx module enriches local feature with the wider range of contextual information  by using contextual branch deep feature. As illustrated in Figure, we first feed a local patch and a context separately to the coding network to obtain local deep feature  $L \in \mathbb{R}^{C \times H \times W}$ and contextual deep feature $C \in \mathbb{R}^{C \times H \times W}$.

% \noindent \textbf{Relative positional embeddings.}
% \textcolor{blue}{Specifically, $\textbf{R}_k$ is passed through a softmax layer to obtain the attention map $\overline{\textbf{R}}_k=\text{Softmax}(\textbf{R}_k)$.}
% (Why we add this?)
However, according to Eq. \ref{eq:m_k1}, $M$ is essentially position-agnostic. It contain insufficient information on how local features $\textbf{X}^I$ and contextual features $\textbf{X}^U$ are spatially correlated, which results in permutation equivariant and thus less expressive for our task. 
To incorporate their position information, one way is to add sinusoidal embeddings based on the absolute position of pixels, but early experimentation suggests that the employment of relative positional embeddings usually results in significantly better accuracies \cite{shaw2018self, ramachandran2019stand}.
% Another possibility is to model the spatial position between pixels with relative positional embeddings.

Therefore, inspired by \cite{d2021convit},
% which [does not ignore the smaller values between in the correlation and positional information to express their relative importance by learnable gating parameters], 
we introduce a gated positional embeddings scheme that adaptively delivers the relative positional information to $M$ via the embeddings $\textbf{r}_{ij}$ of the relative positions of $i$-th and $j$-th patches. To adaptively combine the feature correlation and positional embeddings, the derivation of the attention map $M$ can be expressed as below:
\begin{align}
    M = \text{Norm}( &\sigma(z)\text{Softmax}(\langle\textbf{X}^I,\textbf{X}^U \rangle) \nonumber \\ 
    &+  (1-\sigma(z))\text{Softmax}(\textbf{v}^{T}_{pos}\textbf{r}_{ij})),
    % Gate = (1-\sigma(\lambda))\text{softmax}(\langle\textbf{X}_k^i,\textbf{X}_k^U \rangle)  \nonumber \\
    %  + \sigma(\lambda)\text{softmax}(\textbf{v}^{T}_{pos}\textbf{r}_{ij}),
\end{align}
where $\textbf{v}_{pos}$ ($\textbf{v}_{pos} \in \mathbb{R}^{D_{pos}}$) represent a trainable embedding, and $\textbf{r}_{ij}$ ($\textbf{r}_{ij} \in \mathbb{R}^{D_{pos}}$) denotes the relative positional embeddings computed by the distance of the $i$-th and $j$-th pixel. $\text{Norm}(\cdot)$ normalizes the correlation of the $i$-th pixel and all pixels. Note that, the gating parameter $z$ is trainable and $\sigma(\cdot)$ refers to the sigmoid function, which can dynamically balance the contributions of feature correlation and positional embeddings.
\textcolor{blue}{Last, we use the attention map $M$ to enhance $\textbf{X}^U$ via inner product to yield the locality-aware features, i.e., $\overline{\textbf{X}}^U = \langle M , \textbf{X}^U\rangle$. 
% For the sake of clarity, we denote the entire procedure as $\overline{\textbf{X}}_k = \mathcal{F}_{LCC}(I_k, U_k)$.
}



\subsubsection{Multi-Context Fusion}

% Analogy to the vision system of human being, the contexts of different scales may offer various types of fine-grained details to reason about the content of the local patch. 
% Inspired by the human vision system, the contexts of different scales may provide complementary information to reason the content of local patches. 
For the ultra-high resolution geospatial images that often contain a large number of objects with large size variations, the contexts of different scales may be attributed to the segmentation of the objects with various granularity. 
% But, geospatial images often contain a large number of objects with large contrast in their sizes. 
Therefore, properly combining different contextual information can be complementary for extracting semantics and removing artifacts. 

% to facilitate the segmentation for each patch, 
Specifically, we assume that there are $T$ corresponding context regions that may affect the local segmentation. As shown in the left figure of Fig.~\ref{fig:local_framework}, we have three types of extracted features from large context, medium context, and local context (or local patch) in practice. 
% The routine we choose context regions follows the formulation in Sec.~\ref{sec:choose_context}.
Formally, given the local patch $I$, we have several corresponding context regions, $U_t$ ($t = [1, \cdots, T]$) and pass them into each stream of our local segmentation model to obtain locality-ware features $\overline{\textbf{X}}^{U_t}$. In our practice, $T$ is equal to $3$, and there are three contextual features including local features, medium context features, and large context features. 
% ($\overline{\textbf{X}}_k^t = \mathcal{F}_{LCC}(I_k, U^t_k)$).
% , each of which has a unique dimension, i.e., $(w^{ti}_u, h^{ti}_u) \neq (w^{tj}_u, h^{tj}_u), \forall ti \neq tj$. 

To effectively exploit and combine the locality-aware features that stem from various contexts, as shown in Fig.~\ref{fig:framework}, we integrate a multi-context fusion scheme into our local segmentation model.
% , which adaptively estimates the spatial weight maps for fusing the contextual information in a balanced way. 
% To accomplish this, we first calculate the features enhanced by contexts, i.e., $\overline{\textbf{X}}_k^t = \mathcal{F}_{lcr}(I_k, U_k^t)$, respectively, via the local-context relevance module. 
% a novel network module $\mathcal{F}_{est}$ estimates the weight maps $\{\textbf{H}^t\}$ corresponded to the features $\{\overline{\textbf{X}}^t\}$, respectively.
Specifically, the locality-aware features $\overline{\textbf{X}}^t$ are first concatenated and passed through a \textit{squeeze-and-split} structure, which compresses and entangles the multi-scale features before predicting the normalized weights for the features from different sources, i.e., $\{\textbf{H}^t\} = \mathcal{F}_{est}(\{\overline{\textbf{X}}^{U_t}\})$. $\mathcal{F}_{est}$ refers to the network structure for predicting weights. The squeeze-and-split structure
squeezes the concated features via a convolutional layer with the kernel size $1 \times 1$, which blends the locality-aware features. Then, the squeezed features are reconstructed to the original dimension via another $1 \times 1$ convolutional layer and passed through a softmax to obtain $T$ normalized weight maps $\{\textbf{H}^t\}$ ($\textbf{H}^t \in \mathbb{R}^{h_x \times w_x}$, $t= [1,\cdots,T]$) which balance the contributions of each term. Hence, we have the fused locality-aware features $ {\overline{\textbf{X}}}$ as below:
\begin{align}
    {\overline{\textbf{X}}} &= \sum_{t=1}^T \textbf{H}^t \odot \overline{\textbf{X}}^{U_t}, \quad s.t.  \sum_{t=1}^T \textbf{H}^t = \textbf{1}
\end{align}
where $\odot$ refers to the element-wise multiplication and $\textbf{1}$ represents the matrix where all elements are 1. Note that, the elements of $T$ weight maps along each channel are summed to be 1. 
% Last, the fused features will be joined with the features of the local patch via a skip connection to form a residual structure, and then used to compute the segmentation mask of the patch via several upsampling layers in the decoder.
In this way, our feature fusion scheme is able to take advantage of the complementary information from different contexts.


% the loss function of our local segmentation model is: 
% \begin{align}
%     \mathcal{L}_{seg} = - y(1-p)^\gamma log(p) - (1-y)p^\gamma log(1-p)
% \end{align}



% \subsection{Collaborative Local Representation Optimization}
\subsection{Alternating Local Enhancement}

As mentioned above, our proposed LCF is able to leverage the contextual information to complement the local features, but its non-local correlation scheme inevitably introduces lots of redundant information. Besides, LCF mainly focuses on the fusion of the contextual features, so we treat the contextual features as static features in the training process. Thus, the contextual information is not fully exploited to infer the local semantics. \wxb{To remedy the shortcomings, we propose the alternating local enhancement (ALE) module. We elaborate the ALE in the following. } 
% To remedy the shortcomings, we propose the collaborative local representation optimization module (CLROM). We elaborate the CLROM in the following.  

\subsubsection{Alternating Optimization for Local Features}

% In practice, 
To prevent from bringing in redundant information outside the local region of interest, we need to concentrate on the common region from local patch and contexts.
% First, to avoid the redundant information in the non-local regions, we crop the local area from the contextual features and upsample it to align with the features of local patch. 
As show in Fig.~\ref{fig:framework}, we have the features of the local patch $\textbf{X}^I$, as well as the medium and large context features. Then, we crop their center regions that align with the local patch $I$ and resize them to the same dimension as $\textbf{X}^I$, which are denoted as ${\textbf{X}}^{M}$ and ${\textbf{X}}^{L}$, respectively. Hence, both of them involve the contextual information from the neighboring areas without introducing too much noise.

Next, we want to employ them to jointly infer local semantics. Formally, the objective can be formulated as an non-linear function $f(\cdot)$ that aims to obtain the optimized segmentation results:
\begin{align}
    \hat{\textbf{X}}^{I} = \mathop{\arg\min}_{\textbf{X}^I,\textbf{X}^{M}, \textbf{X}^{L}} f(\textbf{X}^I, \textbf{X}^{M}, \textbf{X}^{L}),
\end{align}
where $f(\cdot)$ refers to a non-linear function w.r.t. three parameters $\textbf{X}^I$, $\textbf{X}^{M}$, and $\textbf{X}^{L}$. Through the optimization, we can leverage their mutual relation to infer the optimal local representation $\hat{\textbf{X}}^{I}$ that can generate high-quality segmentation results.

To solve the optimization, we can apply an alternating optimization technique by iteratively optimizing the function w.r.t. one parameter while freezing the others. Hence, the iterative optimization procedure can be expressed as below:
\begin{align}
    \hat{\textbf{X}}^{large} &= \mathop{\arg\min}_{\textbf{X}^{large}} f(\textbf{X}^{large} ; \textbf{X}^{i}, \textbf{X}^{med}),\\
    \hat{\textbf{X}}^{med} &= \mathop{\arg\min}_{\textbf{X}^{med}} f(\textbf{X}^{med} ; \textbf{X}^{i}, \hat{\textbf{X}}^{large}),\\
    \hat{\textbf{X}}^{i} &= \mathop{\arg\min}_{\textbf{X}^{i}} f(\textbf{X}^{i} ; \hat{\textbf{X}}^{med}, \hat{\textbf{X}}^{large}),
\end{align}
where $\hat{\textbf{X}}^{i}$, $\hat{\textbf{X}}^{med}$, and $\hat{\textbf{X}}^{large}$ are the optimized features. According to the process above, we can design a specific network structure as shown in the right figure of Fig. \ref{fig:local_framework}. As the core of the structure, $f(\cdot;\cdot,\cdot)$ is a specific function block, denoted as local feature interaction (LFI) block, that leverages two reference patches to refine the target patch. We will elaborate the LFI block in the following. 

\subsubsection{Local Feature Interaction}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{imgs/ev.png}
%     \caption{ev...}
%     \label{fig:ev}
% \end{figure}

As mentioned, LFI serves as a function $f$ that aims to utilize two reference patches to strengthen the target patch. Given the spatially-aligned features of the reference patches and target patch cropped from different contexts, they contain the semantic information in different granularity. To avoid introducing redundant information, we confine the pixel-level feature enhancement within small neighboring region. Hence, we design a novel spatial attention model to discover the local relation around each pixel. 


% (Motivation, i.e. why)
% \textcolor{blue}{From the pixel level, the locality-aware contextual correlation module uses all pixels in the context to reconstruct local patch, which may contain redundant information. Therefore, we proposed the local-context interaction module to focus on enhancing the feature of the patch by using the information around the patch,  which contains the restricted context information. We use the locality-confined feature $\textbf{X}_k^c$ cropped from contextual feature and its location is corresponding to the local feature.}

% (comparing to local context)
% \textcolor{blue}{Compared with the local context, the local context uses all the pixels of the context, while $\textbf{X}_k^c$ only uses the features of the neighboring areas of the pixels, which restricted contextual information and reduces redundant information.}

% (Locality-Confined Attention)
% \textcolor{blue}{
Formally, the reference feature patches can be denoted as $\{\textbf{X}_{ref}^1, \textbf{X}_{ref}^2\}$ and the target feature patches are denoted as $\textbf{X}_{tar}$. 
In specific, the target features $\textbf{X}_{tar}$ and the reference features $\textbf{X}_{ref}^i$ ($i=\{1,2\}$) are tokenized via $1\times 1$ convolutional layers. 
The features of the reference patches are first concatenated as $\textbf{X}_{ref} = \text{Concat}\{\textbf{X}_{ref}^1, \textbf{X}_{ref}^2\}$.
Then, 
% To accomplish the locality, 
a 2D kernel $\kappa$ with the size $\omega \times \omega$ can be adopted to convolve the features $\textbf{X}_{ref}$ and derive an attention map $E$ ($E \in \mathbb{R}^{H\times W \times C}$) to strengthen the target features $\textbf{X}_{tar}$. 
% . Thus, by convolving the locality-confined features $\textbf{X}_k^c$ with the kernel $\kappa$, we can derive an attention map $E$ ($E \in \mathbb{R}^{H\times W \times C}$).
% }

Unlike the standard spatial attention module, as illustrated in the network structure on the right part of Fig.~\ref{fig:local_framework}, we adopt kernels with different window sizes, \wxb{to involve feature information of varied granularity.}
% to involve rich contextual information of varied scales. 
To do so, we slice the features $\textbf{X}_{ref}$ along channels into groups and then convolve the features of each group with a distinct 2D kernel via depthwise convolution, denoted as \textit{GroupDepthConv}, which can be expressed as below.
\begin{align}
    E = & \text{GroupDepthConv}_{i = \{1, \cdots, G\}}(\textbf{X}_{ref}; \{c_i\}, \{\kappa_i\}),\nonumber \\
    = & \oplus_{i=1}^G \text{DepthConv}(\textbf{X}_{ref}[c_{i-1}+1:c_i]; \kappa_i),
\end{align}
where $\oplus$ denotes the channel-wise concatenation and $G$ is the number of groups. $c_i$ represents the channel index ($c_i=0$ when $i=0$ and $c_i \in \mathbb{N}^{+}$ otherwise). $\textbf{X}_{ref}[c_{i-1}+1:c_i]$ implies the sliced feature maps of the $i$-th group, ranging from the $(c_{i-1}+1)$-th channel to $c_i$-th channel of $\textbf{X}_{ref}$. $\kappa_i$ refers to the 2D kernel with the size of $\omega_i \times \omega_i$. 
Last, we leverage the estimated attention map $E$ to enhance the target features via a residual structure, i.e.:
\begin{align}
    \overline{\textbf{X}}_{tar} &= \textbf{X}_{tar} + E \odot \textbf{X}_{tar},
\end{align}
where $\overline{\textbf{X}}_{tar}$ is the enhanced target features, and $\odot$ denotes element-wise multiplication. 


% In practice, we evenly separate the channels into eight groups, and set the corresponding kernel sizes as $\{3, 3, 5, 5, 5, 7, 7, 7\}$.

% \textcolor{blue}{
% In order to aggregate effective information from locality-confined patch, we may need to adopt kernels with different window sizes. The main reason is that ..., so they may need to use the kernel with large size, and vice versa. Therefore, we can slice features along channels into groups and then convolve the features of each group with a distinct 2D kernel via a depthwise convolution. Here we denote this operation as group depthwise convolution that can be expressed as below:
% \begin{align}
%     E = & \text{GroupDepthConv}_{i = \{1, \cdots, G\}}(\textbf{X}_k^c; \{c_i\}, \{\kappa_i\}),\nonumber \\
%     = & \oplus_{i=1}^G \text{DepthConv}(\textbf{X}_k^c[c_{i-1}+1:c_i]; \kappa_i),
% \end{align}
% where $\oplus$ denotes the channel-wise concatenation and $G$ is the number of groups. $c_i$ represents the channel index ($c_i=0$ when $i=0$ and $c_i \in \mathbb{N}^{+}$ otherwise). $\textbf{X}_k^c[c_{i-1}+1:c_i]$ implies the sliced feature maps of the $i$-th group, ranging from the $(c_{i-1}+1)$-th channel to $c_i$-th channel of $\textbf{X}_k^c$. $\kappa_i$ refers to the 2D kernel with the size of $\omega_i \times \omega_i$. In practice, we evenly separate the channels into eight groups, 
% and set the corresponding kernel sizes as $\{3, 3, 5, 5, 5, 7, 7, 7\}$.
% }
% \textcolor{blue}{
% Last, we leverage the estimated attention map $E$ to enhance the target features via a residual structure, i.e.:
% \begin{align}
%     \overline{\textbf{X}}_{tar} &= \textbf{X}_{tar} + E \odot \textbf{X}_{tar},
% \end{align}
% }
% \textcolor{blue}{
% where $\overline{\textbf{X}}_{tar}$ is the enhanced target features, and $\odot$ denotes element-wise multiplication. 
% }



% \subsection{Contextual Semantics Refinement Network}



% In prior practices, montaging the computed segmentation masks of all cropped patches easily cause boundary artifacts, so the local masks are stacked together in an overlapping manner (see the third step in Fig.~\ref{fig:steps}) and the results on the overlap regions are computed in average, which somewhat reduces the artifacts. Merging all the local masks in this way eventually leads to the final high-resolution result. 
% However, this trivial approach can hardly achieve the optimal results without adaptively considering the semantic correlation between local patch and its context. To address this issue, we propose a contextual semantics refinement network to exploit contextual semantic mask to refine the local mask.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{imgs/mergenet++.png}
%     \caption{Illustration of contextual semantics refinement network. Given a crude high-resolution semantic mask, we feed a local mask and its context mask into a two-branch network to refine the local mask.}
%     \label{fig:merge}
% \end{figure}

% Given the computed local segmentation masks, we can spawn the crude high-resolution mask via simply montaging local patches or merging masks in an overlapping manner. Although this coarse result may contain artifacts, the semantics from context play the important role to embody the geospatial layout of neighboring regions, and thus facilitate the refinement of the local mask. In specific, as shown in Fig. \ref{fig:merge}, our refinement network bases on a two-stream variant of U-Net architecture which incorporates a local-context relevance module to associate the context and local mask. The local-context relevance module is similar to the locality-aware correlation module in our local segmentation model, which measures the correlation between the features of local mask and context mask that are rescaled to be the same dimension as local mask, and then attentively enhances the local mask. To this end, the contextual semantics can be leveraged to not only remove  the boundary vanishing artifacts but also improve the contours of the local mask.
% Besides, same as the standard U-Net structure, our network bridges the features of the downsampling and upsampling layers via skip connections that deliver low level details to deep layers so as to achieve the refined results. Moreover, we adopt the focal loss as the objective function as well. All the refined local results can be further applied to montage a better quality high resolution semantic mask. 
% \begin{align}
%     \mathcal{L}_{merge} = 
% \end{align}

\subsection{Loss Function}

Last, we apply the focal loss \cite{Lin_2017_ICCV} as the objective function, in which $\gamma$ is set as $3$.

\begin{align}
    & Loss(p_t) = -(1-p_t)^\gamma log(p_t), \\
    & p_t =   \begin{cases}
            p & \text{if} \: y=1 \\
            1-p & \text{otherwise}, \\
            \end{cases}
\end{align}

==> lcf.tex <==
\subsection{Locality-aware Context Fusion}

\wx{*** new version ***}

To strengthen the segmentation of a local patch, we would like to associate the contextual information with the local information. Thus, as illustrated in Fig.~\ref{fig:framework}, apart from any target local patch, we involve two different contexts, the medium context and the large context for estimating the local semantic mask. 
For the sake of simplicity in description, in the following sections, we denote the target local patch as $I$, and their medium and large contexts as $I_M$ and $I_L$.
In the framework, we propose the LCF module $\mathcal{F}_{LCF}$ to evaluate the relevance of the target patch and its contexts, as well as its self-correlation, which are then employed to obtain the locality-aware features of the target patch. 

Concretely, the structure of our produced LCF module is specified in the left figure of Fig.~\ref{fig:local_framework}. It mainly consists of two steps: locality-aware contextual correlation (LCC) and multi-context fusion (MCF). Specifically, LCC discovers the relevance of local patch and contexts to enhance local features, and MCF then adaptively merges them so the contexts can well complement the local features. 

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


